Studying Duplicate Logging Statements and Their Relationships with Code Clones

In this paper, we focus on studying duplicate logging statements, which are logging statements that have the same static text message. We manually studied over 4K duplicate logging statements and their surrounding code in five large-scale open source systems. We uncovered five patterns of duplicate logging code smells. For each instance of the duplicate logging code smell, we further manually identify the potentially problematic and justifiable cases. Then, we contact developers to verify our manual study result. We integrated our manual study result and the feedback of developers into our automated static analysis tool, DLFinder, which automatically detects problematic duplicate logging code smells. We evaluated DLFinder on the five manually studied systems and three additional systems. In total, combining the results of DLFinder and our manual analysis, we reported 91 problematic duplicate logging code smell instances to developers and all of them have been fixed. We further study the relationship between duplicate logging statements, including the problematic instances of duplicate logging code smells, and code clones. We find that 83% of the duplicate logging code smell instances reside in cloned code, but 17% of them reside in micro-clones that are difficult to detect using automated clone detection tools. We also find that more than half of the duplicate logging statements reside in cloned code snippets, and a large portion of them reside in very short code blocks which may not be effectively detected by existing code clone detection tools. Our study shows that, in addition to general source code that implements the business logic, code clones may also result in bad logging practices that could increase maintenance difficulties.

==> Makefile <==

default: paper
	@echo '****************************************************************'
	@echo '**************** Did you spell-check the paper? ****************'
	@echo '****************************************************************'
coall:
	co RCS/*

ciall:
	ci -u *.tex
	ci -u *.eps

bib: paper.bbl

paper.bbl: *.tex paper.bib
	latex paper
	bibtex paper
	latex paper

paper.ps: paper.dvi
	dvips -P cmz paper.dvi -o paper.ps -t letter

paper.dvi: *.tex paper.bbl
	latex paper
	latex paper

paper.pdf: *.tex
	pdflatex paper
	pdflatex paper
mpost:
	mpost -tex=latex overview.mp

paper: *.tex
	pdflatex paper
	bibtex paper
	pdflatex paper
#	pdflatex paper
	#pdf2ps paper.pdf paper.ps

patent: patent.tex
	pdflatex patent

cover: cover.tex
	pdflatex cover
	bibtex paper
	pdflatex cover
	pdflatex cover
	pdflatex cover2

purge:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                paper.ps \
		overview.mps\
		paper.pdf

clean:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                paper.ps




==> texfiles/backup/clone.tex <==
\section{RQ4: What are the Relationships between Duplicate Logging Statements and Code Clone?}
\label{sec:clone}


\phead{Motivation. }
\zhenhao{Comment 2.3, motivation } During our manual analysis in Section~\ref{sec:manual}, we noticed that some duplicate logging statements or duplicate logging code smells may be related to code clones. Code clone or duplicate code is considered a bad programming practice and an indication of deeper maintenance problems~\cite{refactoring1999}.
Prior studies focus on the detection of code clones by applying text-based approaches~\cite{cpminer, kamiya2002} or abstract syntax tree analysis~\cite{baxter1998, jian2007} on program source code. However, these studies did not study code clones from the perspective of logging code. Logging statements might also be copied along with other code since cloning is often performed hastily without much attention on the context~\cite{5463343}. Some cloned logging statements (e.g., the LM logging code smells in Section~\ref{sec:manual}) may fail to correctly record the runtime behaviors; and thus, increase maintenance difficulties.
%Duplicate logging statements may happen by chance (e.g., two different methods share the same error handling mechanism), or may happen due to code clones. Therefore, even if we do not find any duplicate logging code smells, such cloned logging statements may still cause maintenance overhead.

Hence, given the initial observation from our manual study, in this section, we investigate the relationship between duplicate logging statements and code clones. Our finding may provide researchers and practitioners with insights of other possible effects of code clones (e.g., cloned logging statements), how to further improve logging practices, and may inspire future code clone studies. %We conduct our study by answering two research questions.


%Duplicate logging statements may reside in cloned code snippets because code sixth similar syntactics (i.e., cloned code) can be expressed by identical semantic information in log messages (i.e., duplicate logs). However, it is also possible that cloned code, although with similar syntactical structures, may occur in different contexts, therefore is expressed using different semantic information (i.e., different logging statements).

%As shown in previous sections, we observe that some duplicate logging code smells may be related to code clones. Therefore, in this section, we further study the relationship between duplicate logging statements and code clones. Our goal is to empirically study such relationship, provide insights to researchers and practitioners on other possible effects of code clones, and how to further improve logging practice. We conduct our study by answering two research questions. For each RQ, we describe our motivation, approach, result, and followed by a more detailed discussion.

%\jinqiu{Do we miss the rationale behind studying clones and duplicate logging statement? I think the messages are scattered in diff. places.``Code clones are expected to have structural similarities. Duplicate logging statements indicate similar semantic information about program execution. In this or these RQ/RQs, we investigate the relationship between duplicate logging statements and whether the surrounding code snippets are clones. It is possible that duplicate logging statements reside in cloned code snippets because code with similar syntactics could be represented by the same semantic information (i.e., duplicate logs). Meanwhile, it is also possible that clonded code, despite the similar structure, may appear in different contexts, thus should be expressed by different semantic information. Therefore, the fact that duplicate logging statements appearing in cloned code snippets may indicate maintenance issues. Thus, investigating the relationship between syntatic similarity and one indication of semantic similarity (i.e., through logs) can motivate future research in combining these two sources of information or identifying inconsistencies between these two types of similarity due to maintenance challenges."}



%code clone survey: http://research.cs.queensu.ca/home/cordy/Papers/RC_ICPC08_ScenarioEval.pdf


%explore the potentiality of which the study of code clone could help with the problem of duplicate logging statements and further improve the logging practice. %We first illustrate the approach of how we conduct the study, then present the results with discussion.


%Code clone or duplicate code is a bad smell and thus one of the indicators of poor maintainability~\cite{refactoring1999}. If a piece of code is buggy, then the cloned code could also replicate the bug silently. Logging statements might also be copied together with other code since cloning is often performed hastily without much care about the context~\cite{5463343}. This could result in the logging statements fail to correctly logging the runtime behaviors. In this section, we study the relationship between duplicate logging statements and code clone, in order to explore the potentiality of which the study of code clone could help with the problem of duplicate logging statements and further improve the logging practice. We first illustrate the approach of how we conduct the study, then present the results with discussion.


%\phead{RQ4: What is the relationship between duplicate logging statements and code clones?}

%\noindent{\bf Motivation.} In this RQ, we want to further investigate how many duplicate logging statements are indeed related to code clones. The result of this RQ may provide an initial evidence on the prevalence of log-related clones. Our findings may also highlight the issues in maintaining code clones from the perspective of logging statements, and help researchers and developers avoid such problems in the future.

%\zhenhao{This paragraph looks more like the motivation of RQ5} \peter{need to polish: Our results may provide an initial evidence on the prevalence of log-related clones and help researchers and developers avoid such problems in the future.}\peter{TODO: revisit the motivations after the results are done}

%\jinqiu{The result may highlight the issues in maitaining code clones from the aspect of logging statements. Future research in code clone study may consider logging statements to provide developers with better support.}

%Code clone or duplicate code is a bad smell and thus one of the indicators of poor maintainability~\cite{refactoring1999}. If a piece of code is buggy, then the cloned code could also replicate the bug silently. Logging statements might also be copied together with other code since cloning is often performed hastily without much care about the context~\cite{5463343}. This could result in the logging statements fail to correctly logging the runtime behaviors. In this research question, we would like to investigate the relationship between duplicate logging statements and cloned code snippets. We expect to provide an inspiration of how ... \zhenhao{selling point}
%{\em et al$.$}
\noindent{\bf Our approach of mapping code clones to duplicate logging statements.}
We use both an automated and a manual approach to study the relationship between code clones and duplicate logging statements. Due to the large number of duplicate logging statements in the studied systems, we first leverage automated clone detection tools to study whether these logging statements reside in cloned code. In particular, we use NiCad5~\cite{nicad} as our clone detection tool. NiCad5 uses hybrid language-sensitive text comparison to detect clones. We choose NiCad5 because, as found in prior studies~\cite{nicad,NicadEvaluation}, it has high precision (95\%) and recall (96\%) when detecting near-miss clones (i.e., code clones that are very similar but not exactly the same) and is actively maintained (latest release was in July 2019). %We choose NiCad5 because it is capable of detecting near-miss clones with high precision and recall which is at least as well as existing techniques, while it is more flexible that it does not require compiled code~\cite{ROY2009470,nicad}. \zhenhao{In that evaluation of clone detection papers, they didn't say Nicad is the best or better than other tools. They just provided an intention that we could use different tools in different situations, though the situation that Nicad is recommented is not too much of our business.}

In NiCad5, the source code units of comparison are determined by partitioning the source code into different granularities. %a set of disjoint fragments (e.g., methods or code blocks).
%These source code units are the largest source code fragments (e.g., basic blocks) that are considered in the clone detection~\cite{nicad}. %may be clone targets involved in direct clone relations with each other~\cite{nicad}.
The structural granularity of the source code units could be set as the method-level or block-level (e.g., the blocks of {\em catch}, {\em if}, {\em for}, or {\em method}, etc). In our study, we set the level of granularity to block-level and use the default configuration (i.e., similarity threshold is 70\% and the minimum lines of a comparable code block is 10),
%\jinqiu{Does the paper say the default configurations would yield better results? If so, add that here. Intuitively, 10 sounds too big a number for this configuration though. The example of IL in Table 2 does not have more than 10 lines}
which is suggested by prior studies indicating this configuration could achieve remarkably better results in terms of precision and recall~\cite{EvaluatingModernCloneDetectionTools, ROY2009470, nicad}. Block-level provides finer-grained information, since logging statements are usually contained in code blocks for debugging or error diagnostic purposes~\cite{Fu:2014:DLE:2591062.2591175}. Note that if the block is nested, the inner block is listed twice: once inside its parent block and once on its own. Hence, all blocks with lines of code above the default threshold will be compared for detecting clones. %\peter{I moved the numbers above. We can define what they meant by threshold above as well}For the thresholds and settings of detection, we keep them in default (the minimum lines of a comparable block is 10, the similarity threshold is 70\% \zhenhao{might briefly explain how do they define similarity.})\zhenhao{These are the threshold they used, but didn't describe the reasons in their paper}.
%\peter{avoid passive voice}The study is conducted by answering two research questions. For the identification of cloned code, We use NiCad5 to conduct the detection of code clone. NiCad5 is a flexible hybrid language-sensitive text comparison clone detection tool originally based on the previous work of Roy. {\em et al$.$}~\cite{nicad} with continuously maintainence and improvement afterwards. Up to the submission of this work, the latest version of NiCad5 was released on Oct. 05, 2018. The source unit of comparison are determined by partitioning the source into a set of disjoint fragments. These units are the largest source fragments that may be involved in direct clone relations with each other~\cite{nicad}. The structural granularity of source units could be set as method-level or block-level (e.g., the blocks of {\em catch, if, for, method, etc}). In our study, we set the level of granularity as block-level, a more fine-grained level which might provide us with more accurate results. Note that if the block is nested, the inner block is listed twice: once inside its parent block and once on its own. \peter{Hence, all qualified blocks will be compared by the tool.}%So that all the qualified blocks (with more potential cloned lines than the threshold) could be compared.
We run NiCad5 on the eight studied open source systems that are mentioned in Section~\ref{sec:results}. We then analyze the clone detection results and match the location of the clones with that of the duplicate logging statements. If two or more cloned code snippets contain the same set of duplicate logging statements (i.e., the static text messages are the same), we consider the logging statements are related to the clone and record the code clone similarity score.

%\zhenhao{CSD:4, CS:119, ES:5, HD:7, CM:113, FLK:25, KFK:6, WKT:2, Total: 281}
%\zhenhao{272/281, 9 FPs}


Although NiCad5 has a great precision in detecting clones (its precision is 96.8\% in our studied dataset, more details in Section~\ref{sec:threats}), there may still exist some false negatives. Therefore, we then manually investigate a sample of duplicate logging statements which reside in code snippets that are {\em not} classified by NiCad5 as clones. Our goal is to study if these duplicate logging statements are indeed not in cloned code, or they are not detected due to other reasons, e.g., limitation of the clone detection tool NiCad5. We follow similar steps as described in Section~\ref{sec:manual} in our manual analysis. We randomly sample sets of duplicate logging statements that are {\em not} classified by NiCad5 as clones, based on a confidence level of 95\% and a confidence interval of 5\%. Then, we study their surrounding code.



\begin{table}
    \caption{Automated code clone analysis results on duplicate logging statements. {\sf DupSet}: Total sets of duplicate logging statements. {\sf CloneSet}: Sets of duplicate Logging statements that are from cloned code snippets.  {\sf Avg. Sim.}: Average similarity of the cloned code snippets.
}


    \vspace{-0.3cm}
    \centering
    %\resizebox{\columnwidth}{!} {
    \tabcolsep=18pt
    \scalebox{0.8}{

    \begin{tabular}{l|c|c|c}

        \toprule
        & \multicolumn{1}{c|}{\textbf{DupSet}} & \multicolumn{1}{c|}{\textbf{CloneSet}}  & \multicolumn{1}{c}{\textbf{Avg. Sim.}} \\

        \midrule
        \textbf{Cassandra}     & 46  & 14 (30.4\%) & 79.7  \\
        \textbf{CloudStack}     & 865  & 442 (51.1\%) & 80.3  \\
        \textbf{ElasticSearch}  & 40  & 17 (42.5\%) & 72.2  \\
        \textbf{Hadoop}         & 217  & 25 (11.5\%) & 76  \\
        \textbf{Camel}         & 886  & 421 (47.5\%) & 80.7  \\
        \textbf{Flink}         & 203  & 92 (45.3\%) & 78.8 \\
        \textbf{Kafka}         & 104  & 23 (22.1\%) & 75.4  \\
        \textbf{Wicket}         & 21  & 8 (38.1\%) & 83.1 \\
\midrule
        \textbf{Overall}         & 2,382   & 1,042 (43.7\%) & 80.0  \\
        \bottomrule
    \end{tabular}
    }%}
    \vspace{-0.6cm}
\label{table:RQ4}
\end{table}


\begin{comment}
Cloudstack: Y40 H7, 94
Hadoop: Y15 H7, 43
Elasticsearch: Y2, 5
Cassandran: Y3 H1, 7
Camel: Y45 H13, 103
Wicket: H1, 3
Kafka: Y8 H2, 18
Flink: Y8 H1, 25
Total: Y121 H28, 298
\end{comment}

\peter{I wonder if we should put the first part of RQ4 (both automated and manual) in appendix. The motivation would be stronger if we start directly with problematic instances.}
\noindent{\bf Results of automated code clone analysis on duplicate logging statements.} {\em We find that a significant number of duplicate logging statements (43.7\% on average) reside in cloned code snippets.}
Table~\ref{table:RQ4} presents the results of our code clone analysis. {\sf DupSet} refers to the total sets of duplicate logging statements (a set contains two or more logging statements with the same text message). {\sf CloneSet} refers to the subset of duplicate logging statement sets ({\sf DupSet}) that are from cloned code snippets. The percentage number is the proportion of {\sf CloneSet} out of {\sf DupSet}. Finally, {\sf Avg. Sim.} refers to the average code clone similarity score among the cloned code snippets. As shown in Table~\ref{table:RQ4}, 11.5\% to 51.1\% sets of duplicate logging statements are from the cloned code snippets in the studied systems. Overall, 1,042 out of 2,382 (43.7\%) sets of duplicate logging statements are related to code clones (with an average 80\% similarity score).

Our finding shows that a significant number of duplicate logging statements are related to code clones, and developers may not change the log messages when they copy a piece of code to another location.
However, due to the importance of logging for understanding system runtime behaviour~\cite{petericseseip2017, Yuan:2012:CLP:2337223.2337236, Yuan:2011:ISD:1950365.1950369}, developers should avoid directly copying logging statements. Developers should consider modifying the log messages (e.g., to include the class name, modify the message to reflect code changes, or record new important dynamic variables) to assist debugging and workload understanding.

%the proportion in the studied systems varies from 11.5\% to 51.1\%. However, overall 1042 out of 2382 (43.7\%) sets of duplicate logging statements are marked as from cloned code with an average similarity of 80 (i.e., 80\% of the compared source code units are identical in the corresponding blocks. \zhenhao{Need to explain similarity in approach} ).


\noindent{\bf Results of manual code clone analysis on duplicate logging statements.} {\em We find that more than 50\% of the sampled duplicate logging statements reside in cloned code snippets that are difficult to detect using automated code clone detection tools. In particular, 24.5\% of the manually studied duplicate logging statements are related to code clones, and 26.2\% are related to micro-clones. }
In total, we randomly sample 298 sets of duplicate logging statements to achieve a confidence of 95\% and a confidence interval of 5\%. For each set of the sampled duplicate logging statements, we manually classify them into three types if they meet the described criteria:

%We follow similar steps as described in Section~\ref{sec:manual} in our manual analysis. We first randomly sample 298 sets of duplicate logging statements from duplicate logging statements reside in code snippets that are {\em not} classified by NiCad5 as clones (with a confidence level of 95\% and a confidence interval of 5\%). Then, we study their surrounding code. For each set of the sampled duplicate logging statements, we manually classify them into three types if they meet the described criteria:

%\zhenhao{What if we say the threshold of manual study is 10 here? And change the label of those fewer than 10 lines from Clones to Undecideable. Then we discuss why those longer than 10 lines were not detected, and say what we find in the Undecidable ones...}\peter{that would work, but would that require a lot of additional work?}
%\zhenhao{Hmm... not a lot of additional works, as long as doing so is reasonable / correct}
%\peter{but that is still bias towards the threshold. }
%For the duplicate logging statements that are not detected as from cloned snippets, we investigate whether they are truely not from cloned snippets, or they are from cloned snippets but failed to be detected due to some reasons (e.g., limitation of the tool, complicated code structure, etc.). We randomly sample 298 sets of duplicate logging statements with their surrounding code blocks and manually study them following similar phases as described in Section~\ref{sec:manual}. The results of this phase have a Cohen’s kappa of X, which is a Y-level of agreement~\cite{kappa}. For each item of the sample, We manually mark it as one of the following three labels:

\begin{itemize}\itemsep 0em
    %\item Clones (C): if at least two of the logging statements in the set meet the following requirements: 1) The surrounding code block that the logging statement locates in has 5 or more lines of code. \zhenhao{the reason is, it's hard to say if short blocks are clones or just by chance.} 2) At least 5 lines of code surrounding the logging statement are exactly the same, or nearly the same, only with the differences of identifier names.
    \item Clones: %1) The code block where the logging code statements are located is not too short (i.e., has ten or more lines of code, consistent with the threshold of the tool). 2)
    The code around the logging statements is more than 10 lines of code (same as the threshold of the clone detection tool). The code is exactly the same, or only with differences in identifier names (i.e., Type 1 and Type 2 clones~\cite{CompareCloneDetectionTools2007}) while not detected by the automated clone detection tool.

    \item Micro-clones: The code around the logging statements is very similar but is less than 10 lines of code~\cite{microclones}. Prior studies show that micro-clones are more difficult to detect due to their size. However, the effect of micro-clones on code maintenance and quality is similar to regular-size clones~\cite{MicroclonesAndBugsICPC, MicroclonesAndBugsSANER}. Micro-clones should not be ignored when making decisions of clone management.
     %1) The code block where the logging code statements are located is short (i.e., has fewer than ten lines of code\peter{might need to remove the rest?}, below the threshold of the tool). 2) The code in the block is exactly the same, or only with differences in identifier names. For this kind of situations, though we feel they are likely to be clones, their sizes are not long enough for us to make a decision. Therefore, we label them as "Undecidable".
     %Prior studies indicate that micro-clones have similar tendencies of replicating severe bugs as regular clones~\cite{MicroclonesAndBugsICPC, MicroclonesAndBugsSANER}.
     \item Non-clones: For other situations, we mark them as non-clones.
\end{itemize}


%The columns under ``DupSet'' in
Table~\ref{table:manualrq4} presents the results of our manual study. Overall, 73 out of the 298 (24.5\%) manually-studied sets of duplicate logging statements are labeled as {\em Clones}. 78 out of 298 (26.2\%) sets are labeled as {\em Micro-clones}. The remaining 147 out of 298 (49.3\%) sets are labeled as {\em Non-clones}.
%The proportion of {\em Clones} that we observe in the manual study (40.1\%) is similar to the clones that are detected by the tool (43.7\%). \zhenhao{Need to apply the new threshold and update the results.}~\jinqiu{I do not think the porportion means much though, we can just say the percentage of agreed results on the `clone' labels between the manual work and the clone tool.}
For the clones and micro-clones that are identified by our manual analysis but not detected by the tool, we summarize the potential reasons into three categories. Note that the tool may fail to detect a clone due to one or more reasons.

{\em \underline{Category 1:} Code clones reside in part of a large code block.} Since the structural granularity level of the source code units is block-level (i.e., the minimal comparable source code unit of the tool is a block), the similarity of the code is computed by comparing blocks. However, for 42 out of the 73 cases of {\em Clones}, and 32 out of 78 cases of {\em Micro-clones}, we find that developers often only copy and paste part of the code into another large code block. For example, developers may copy the code (along with the logging code statements) that is related to establishing network connect from one file to another. However, the copied code is just part of another complex method; hence, the clone detection tool fails to detect the code snippets as clones since the minimum detectable source code unit is block.

%{\em \underline{Category C-1:} Code clones reside in part of a large code block.} Since the structural granularity level of the source code units is block-level (i.e., the minimal comparable source code unit of the tool is a block), the similarity of the code is computed by comparing blocks. However, for 42 out of the 73 sampled cases, we find that developers often only copy and paste part of the code into another large code block. For example, developers may copy the code (along with the logging code statements) that is related to establishing network connect from one file to another. However, the copied code is just part of another complex method; hence, the clone detection tool fails to detect the code snippets as clones.

{\em \underline{Category 2:} Code clones reside in code with very similar semantics but have minor differences.}  %\peter{do you know if they are Type 1, 2, or 3 based on the definition?} \zhenhao{for this category some are type 2 some are type 3. They claim they can detect type 1 - 3 clones in the paper, but idk why some type 2, 3 clones were not detected even though the blocks were longer than 10 lines.}
For 53 out of the 73 cases that are manually identified as {\em Clones}, we find that the surrounding code of duplicate logging statements share highly similar semantics (i.e., implement a similar functionality), but have minor differences (e.g., additions, deletions, or partial modification on existing lines). Such scattered modifications might significantly reduce the similarity between the code structures, and thus, result in miss detection~\cite{ROY2009470,nicad}. %Note that in some cases, they are characterized as belong to both of the two reasons (i.e., they reside in part of a long code block, and with slight modifications).
For example, there is a code block in {\tt\small \textbf{FTP}Consumer} of Camel which does a series of operations based on the file transfer protocol (FTP). %The code in the block may be reuseable for other similar ptopocols. Thus,
Due to the similarity between FTP and secured file transfer protocol (SFTP), Camel developers copied the code block and made modifications (e.g., change class and method names) to the all the places where SFTP is needed (e.g., {\tt\small \textbf{SFTP}Consumer}). Therefore, clone detection tools may fail to detect this kind of cloned code blocks as due to minor yet scattered changes.
%\jinqiu{What about the opposite side? The dupSets are not in code clones. DupSets cannot always be detected by clone tools. Many dup. logging statements are not due to structural similarity but flow similarity??}

{\em \underline{Category 3:} Short methods.}
For more than half of the cases that are labeled as {\em Micro-clones} (46 out of 78), we find that these logging statements reside in very short methods with only a few lines of code. For example, there is a method in CloudStack named {\em verifyServicesCombination()} containing only six lines of code and duplicately locates in three different classes. The method verifies the connectivity of services, and generates a warning-level log if it fails the verification. Clone detection tool fails to detect this category of cases due to their small size compared to regular methods.


%For the cases that are identified as undecidable in our manual study, we categorize them into two categories.

%{\em \underline{Category 3:} Short methods.}
%For more than half of the cases that are labeled as {\em Micro-clones} (46 out of 78 cases), we find that these logging statements reside in very short methods with only a few lines of code. For example, there is a method in CloudStack named {\em verifyServicesCombination()} containing only six lines of code and duplicately locates in different classes. The method verifies the connectivity of services, and generates a warning-level log if it fails the verification. In such situations, although we suspect that two code snippets are clones, it is also possible that the code is the same by coincidence.% since short methods do not execute considerable system behaviours.

%{\em \underline{Category U-2:} Short code blocks within a larger code block.} % reside in long parent blocks.}
%For 32 out of 78 cases, we find that the logging statements are located in short code blocks (e.g., {\em catch} blocks in exception handling), but such code blocks are located within a larger code block.
%For example, there are two different application deployment approaches in Kafka, located in two classes: {\tt\small ConnectStandalone} and {\tt\small ConnectDistributed}. Both of the classes contain {\em catch} blocks that abort the system and record an error message when an exception happen. Even though the code in the catch blocks is exactly the same, the code in the {\em try} blocks is different (i.e., process different deployment types). Hence, it is difficult to say that the code in the {\em catch} blocks is clone. %not identified as code clones by the clone detection tool and is difficult to.
%Moreover, the exception handling code and log messages in such cases may be generic, so it is possible that developers intentionally write the same code for exception handling. %this sort of identical code snippet, rather than copy-and-paste.


%and the rest part of their parent blocks are noticeably different, they are omitted by the clone detection tool. For example, there are two application deployment methods in Kafka, located in Class ConnectStandalone and Class ConnectDistributed, respectively. Both of them contain catch blocks which abort the system and log an error message when an exception happen. Though the code in catch blocks are exactly the same, the code in their parent blocks are different (they process the deployments in different types), they are not detected by the clone detection tool.
%Moreover, the exception handling code and log messages in this kind of situation might be in general. Hence, it is possible that developers intentionally write this sort of identical code snippet, rather than copy-and-paste.

\rqboxc{We find that more than half of the duplicate logging statements reside in cloned code snippets. Our manual study also highlights that many duplicate logging statements reside in cloned code that may be difficult to detect.}



\begin{table}
  \caption{The result of manual study on duplicate logging statements and code clones.}
    \vspace{-0.3cm}
    \centering
    %\resizebox{\textwidth}{!} {
    \tabcolsep=8pt
    \scalebox{0.9}{
    \begin{tabular}{l|cccc}

        \toprule
     &{\textbf{Clones}} &{\textbf{Micro-clones}} &{\textbf{Non-clones}} &{\textbf{Total}}  \\
\midrule

        \textbf{Cassandra}    & 1 & 3 & 3 & 7  \\
        \textbf{CloudStack}    & 22 & 26 &46  & 94 \\
        \textbf{ElasticSearch} & 1 & 1 & 3 & 5 \\
        \textbf{Hadoop}      & 12 & 6 & 25  & 43 \\

       \textbf{Camel}       & 28 & 30 & 45 & 103 \\
       \textbf{Flink}       & 5 & 4 & 16 & 25\\
       \textbf{Kafka}       & 3 & 7 & 8 & 18 \\
       \textbf{Wicket}       & 1 & 1 & 1 & 3 \\

        \midrule

        \textbf{Total}       & 73 &78 & 147 & 298 \\


        % cass non-dup median 7, 0.146 neg
        % cloud stack non-dup median 8, 0.045 neg
        % es non-dup median 7, 0.27 small
        % hadoop non-dup median 6, 0.08 neg
        \bottomrule
    \end{tabular}}
    %}
    \vspace{-0.3cm}

    \label{table:manualrq4}
\end{table}



%\phead{RQ5: What is the relationship between the problematic instances of duplicate logging code smells and code clones?}
\phead{Discussion: Studying the relationship between problematic instances of duplicate logging code smells and code clones.} %As discussed in the previous sections, not all of the duplicate logging code smells are problematic and require fixes. While non-problematic duplicate logging statements may be an indication of maintenance problem, problematic instances of duplicate logging code smells should be fixed in order to correctly record the execution behaviors. Hence, On top of the study on duplicate logging statements and code clones,
\peter{we can merge table 8 and 9 together to avoid confusion. We can say directly that we use tool assisted manual study}We further analyze our clone detection results to investigate how many {\em problematic instances} of duplicate logging code smells are related to code clones. We use the automated clone detection results obtained in this RQ and match them with problematic instances of logging code smells. To reduce the effect of false negatives, we manually study the code of {\em all} the remaining instances that are not identified as clones. % For the instances that are not identified by NiCad5 as code clones (i.e., potential false negatives) \zhenhao{I'm still feeling this should be false negatives. In my understanding, positive = alarm = detected}\peter{you are right...I made a mistake here}, we manually study {\em all} of them to reduce the effect of false positives on the result.%match the results with the instances of problematic duplicate logging code smells that are studied in Section~\ref{sec:manual} and \ref{sec:results}. We then manually study {\em all} the instances of problematic duplicate logging code smells residing in code snippets that are {\em not} classified by NiCad5 as clones (i.e., false positives).

%\noindent{\bf Motivation.}
%In RQ4 we conduct an investigation of the relationship between duplicate logging statements and code clones. However, As discussed in the previous sections, not all of the duplicate logging code smells are problematic and require fixes. While non-problematic duplicate logging statements may be an indication of maintenance problem, problematic instances of duplicate logging code smells should be fixed in order to correctly record the execution behaviors. Thus, in this RQ, we would like to specifically investigate how many problematic instances of duplicate logging code smells are related to code clones and the potential impact of code clones on logging practice.

%\noindent{\bf Approach.}
%We use the clone detection results obtained in RQ4 and match the results with the instances of problematic duplicate logging code smells that are studied in Section~\ref{sec:manual} and \ref{sec:results}. We then manually study {\em all} the instances of problematic duplicate logging code smells residing in code snippets that are {\em not} classified by NiCad5 as clones.



\begin{table*}
  \caption{The result of automated code clone analysis on problematic instances and code clones.  {\sf Num. Ins.} shows the number of problematic code smell instances. {\sf Cloned. Ins.} shows the number of problematic code smell instances that are detected as clones.  {\sf Sim.} shows the average similarity of the cloned code snippets.}
    \vspace{-0.3cm}
    \centering
    %\resizebox{\textwidth}{!} {
    \scalebox{0.78}{
    \tabcolsep=8pt
    \begin{tabular}{c|rrr|rrr|rrr|rrr}

        \toprule
    & \multicolumn{3}{c|}{\textbf{IC}} & \multicolumn{3}{c|}{\textbf{IE}} & \multicolumn{3}{c|}{\textbf{LM}} & \multicolumn{3}{c}{\textbf{DP}}\\
    & Num. Ins. & Cloned. Ins. &Sim. & Num. Ins. & Cloned. Ins. &Sim.& Num. Ins. & Cloned. Ins. &Sim.& Num. Ins. & Cloned. Ins. &Sim. \\
\midrule

        \textbf{Cassandra}     & 1 & 0 (0\%) & --    & 0 & -- (--)  &--     & 0  & -- (--)  &--  & 2&  2 (100\%) &70 \\
        \textbf{CloudStack}    & 8 & 5 (62.5\%) &72.6    & 4 & 4 (100.0\%)  &99     & 27& 20 (74.1\%)  &77.4  &  107 & 60 (56.1\%) &77 \\
        \textbf{ElasticSearch} & 1 & 0 (0\%)  &--    & 0 &-- (--)  &--     & 1  & 0 (0\%)  &--  & 3& 0 (0\%) &-- \\
        \textbf{Hadoop}        & 5 & 1 (20\%)  &70    & 0 &-- (--)  &--     & 9 & 0 (0\%)  &--  & 27& 5 (18.5\%) &70.4 \\

       \textbf{Camel}         & 1 & 0 (0\%) &--     & 0 & -- (--) & --      & 14  & 6 (42.9\%)  &75.2  & 29 & 22 (75.9\%) &72.5 \\
       \textbf{Flink}         & 0 & -- (--)  &--    & 2 & 1 (50.0\%)  & 80     & 4  & 2 (50\%)  &75  & 24 & 19 (79.2\%) &81.7 \\
       \textbf{Kafka}         & 0 & -- (--)  &--    & 0 & -- (--)  &--      & 3  & 1 (33.3\%)  &95.0  & 14 & 3 (21.4\%) &74 \\
       \textbf{Wicket}         & 1 & 0 (0\%) &--     & 0 & -- (--) &--     & 1  & 0 (0\%)  &--  & 1 & 1 (100\%) &100 \\

        \midrule

        \textbf{Total}         & 17 &6 (35.3\%) & 72.2     & 6 & 5 (83.3\%) &95.2     & 59 &29 (49.2\%) &77.4     &207 & 112 (54.1\%) &76.6\\


        % cass non-dup median 7, 0.146 neg
        % cloud stack non-dup median 8, 0.045 neg
        % es non-dup median 7, 0.27 small
        % hadoop non-dup median 6, 0.08 neg
        \bottomrule
    \end{tabular}
    }
    %}
    \vspace{-0.3cm}

    \label{table:RQ5}
\end{table*}

%\peter{You can use multirow to make the second part of the sentence in the next line. Then in the text, we just say, the first column shows...}
%\noindent{\bf Quantitative study.}
\noindent{\bf Result of automated code clone analysis on problematic instances.}
{\em We find that more than half of the problematic instances of duplicate logging code smells (52.6\%) reside in cloned code snippets.}
Table~\ref{table:RQ5} presents the results of our automated code clone analysis. The term {\sf Num. Ins.} refers to the number of instances of problematic duplicate logging code smells. {\sf Cloned. Ins.} refers to the number of problematic instances that are identified by NiCad5 as in code clones. The percentage following each number indicates the proportion of {\sf Cloned. Ins.} out of {\sf Num. Ins}. {\sf Avg. Sim.} refers to the average similarity of {\sf Cloned. Ins}. As shown in Table~\ref{table:RQ5}, 6 out of 17 (35.3\%) instances of IC, 29 out of 59 (49.2\%) instances of LM, 5 out of 6 (83.3\%) instances of IE, and 112 out of 207 (54.1\%) instances of DP are identified as from cloned code snippets.

{\em Overall, we find that many instances (i.e., IC, IE, LM and DP) of problematic duplicate logging code smells (152 out of 289) are related to code clones}. In other words, in addition to the finding from prior code clone studies which indicates that code clones may introduce subtle program errors~\cite{contextCloneBugs, tracyhallcodesmell}, {\em we find that code clones may also result in bad logging practices that could increase maintenance difficulties.} Future studies should further investigate the negative effect of code clones on the quality of logging statements and provide a comprehensive logging guideline.
%\jinqiu{Is IE somehow special and worth a brief discussion?}
%\zhenhao{Hmm the size of IE is too small compared to other patterns.}
%\jinqiu{is it interesting to differenciate type i and type ii clones?}
%\zhenhao{The tool doesn't specify the type in the report.}
%Our results shed light on the potential effects of code clones on other aspects of source code (i.e., logging).~\jinqiu{Is this identical text with that of RQ4? We can be more specific here: due to the problematic nature, more or less related to code clones?} Future studies should further study how code clones may affect debugging production problems and program comprehension.
%program comprehension  %shows that many logging-related issues are related to code clones.

\begin{comment}
\peter{maybe can comment this part out. this is discussed in the discussion}The proportion of clones in IC is lower than that of other patterns. The potential reason might be that the instances of IC are located in different catch blocks of the same try block. Based on our observation during the manual study, the code in catch block is usually short, with only a few lines of exception handling code. Thus, the code is often omitted by clone detection tools which requires a larger code block. %takes a non-negligible number of the minimum lines of comparable source code into account.
Technically it is hard to identify whether the surrounding code of IC instance is from cloned code or not.

%show that most of the problematic logging code smell instances are related to code clones.
\end{comment}



\begin{table*}
  \caption{The result of manual study on problematic instances and code clones. {\sf IC, IE, LM, DP}: Instances of each pattern.}
    \vspace{-0.3cm}
    \centering
    %\resizebox{\textwidth}{!} {
    \tabcolsep=5pt
    \scalebox{0.83}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc}

        \toprule
      & \multicolumn{3}{c|}{\textbf{IC}} & \multicolumn{3}{c|}{\textbf{IE}} & \multicolumn{3}{c|}{\textbf{LM}} & \multicolumn{3}{c}{\textbf{DP}} \\
   &Clones &Micro-clones & Total &Clones &Micro-clones & Total &Clones &Micro-clones & Total &Clones &Micro-clones & Total \\
\midrule

        \textbf{Cassandra}    & 0 & 0 & 1     & 0  &0  & 0     & 0 & 0 & 0     &  0  &0 &0 \\
        \textbf{CloudStack}      & 0  &3 & 3    & 0 &0 & 0    & 1  &5 & 7     & 12 &9 &47 \\
        \textbf{ElasticSearch}    & 0 & 0 & 1      & 0 &0  & 0   &0  &1  & 1       & 1  &0  &3\\
        \textbf{Hadoop}          & 0  &2 & 4     & 0 &0  & 0   &3  &3  & 9       & 14  &6  &22\\

       \textbf{Camel}          & 0 &1 & 1     & 0  &0 & 0    & 2 & 6 & 8      &2 &4  &7\\
       \textbf{Flink}           & 0 &0 & 0     & 0 &1 & 1    & 0 & 2 & 2       &0  & 3 &5\\
       \textbf{Kafka}           & 0  &0 & 0    & 0 &0 &0    & 0  &1  &2     & 3 & 2 &11 \\
       \textbf{Wicket}           & 0 &0 & 1       & 0 &0 & 0     & 1 &0  &1          & 0 &0  &0 \\

        \midrule

        \textbf{Total}           & 0 &6 & 11    & 0 &1  &1     & 7 & 18 &30         &32 &24 &95\\


        % cass non-dup median 7, 0.146 neg
        % cloud stack non-dup median 8, 0.045 neg
        % es non-dup median 7, 0.27 small
        % hadoop non-dup median 6, 0.08 neg
        \bottomrule
    \end{tabular}}
    %}
    \vspace{-0.3cm}

    \label{table:manualrq5}
\end{table*}



%\noindent{\bf Manual study.}
\noindent{\bf Result of manual code clone analysis on problematic instances.}
{\em We find that 64.2\% of the problematic instances of duplicate logging code smells 
%reside in cloned code snippets that are difficult to detect using automated clone detection tools.
that are labeled as Non-clones by the automated code clone detection tool are actually from cloned code snippets.
Among them, more than half (55.7\%) reside in micro-clones which often do not get enough attention in the process of code clone management.}
%Comment 1.6: 64.2\% = numbers in table 9 (all the clones + all the micro-clones)/total
%Comment 1.6: 55.7\% = micro clones / total

%In our clone detection result, we find that only 49.2\% of LM are identified as from cloned code snippets. Based on our manual analysis in previous sections, we find that many LM instances are related to copy-and-paste code, so we expect that more LM instances would be related to code clones. As a result, for the instances that are {\em not} detected as from cloned snippets, we further conduct a manual study on whether they are actually not from cloned code snippets, or the clone detection tool fails to detect them. We follow a similar process that we discuss in the previous part of this section. We manually study {\em all} the problematic instances that are not detected as from cloned code snippets (137 instances in total) and their surrounding code.
%Note that for the instances of IC, since they are in catch blocks of the same try block which are often very short, we mark them as clones if the code in the catch blocks are exactly the same, in spite of how many lines of code they have.
%The columns from ``IC'' to ``DP'' in
We manually study {\em all} the problematic instances (and their surrounding code) that are not detected as from cloned code snippets (137 instances in total). Table~\ref{table:manualrq5} presents the results of our manual study for each pattern. We categorize each instance according to the labels that we discuss earlier in this RQ (i.e., Category 1-3). Below, we describe the results of each pattern followed by a more detailed discussion.

\noindent{\bf {\em IC \& IE: }} {\em 58\% of the IC and IE instances are related to micro-clones.} Since both of IC and IE reside in {\em catch} blocks, which usually contain only a few lines of code, we discuss these two duplicate logging code smells together. As shown in Table~\ref{table:manualrq5}, none of the IC and IE instances are labeled as {\em Clones}, while 7 (6 IC + 1 IE) out of 12 (11 IC + 1 IE) instances are labeled as {\em Micro-clones}. The remaining five instances are single logging statement that might be thrown with multiple types of exceptions (e.g., {\sf catch (Exception1 \(|\)  Exception2 e)}). We find that all of the seven {\em Micro-clones} instances belong to Category 1 (i.e., short code snippets within a large code block). The reason might be that these logging statements all reside in {\em catch} blocks, which are usually very short. Thus, although the code in these short code blocks are identical or highly similar, they are not long enough to be considered as comparable code blocks by the clone detection tool. %Their parent blocks may have sufficient length, but the cloned code only occupies a small portion of their parent blocks. Thus, the tool fails to detect them due to the insignificant similarity of their parent blocks.
%\peter{not sure if we still want to keep this}Compared to clone detection tools, since \toolS analyzes the code in the {\em catch} blocks using static analysis, \toolS is able to detect both IC and IE with very high precision and recall.

%\noindent{\bf {\em IC \& IE: }} Since both of IC and IE reside in {\em catch} blocks, which usually contain only a few lines of code, we discuss these two duplicate logging code smells together. As shown in Table~\ref{table:manualrq5}, none of the IC and IE instances are labeled as Clones, while 7 (6 IC + 1 IE) out of 12 (11 IC + 1 IE) instances are labeled as Micro-clones. The remaining 5 instances are single logging statement that might be thrown with multiple types of exceptions (e.g., {\sf catch (Exception1 \(|\)  Exception2 e)}). We find that all of the seven Micro-clone instances belong to Category 1 (i.e., short code snippets within a large code block, discussed in RQ4). The reason might be that these logging statements all reside in {\em catch} blocks, which are usually very short. Thus, though the code in these short code blocks are identical or highly similar, it is difficult to determine whether they are code clones or due to the fact that code can be repetitive, especially in smaller code blocks~\cite{naturalness}. Compared to clone detection tools, since \toolS analyzes the code in the {\em catch} blocks using static analysis, \toolS is able to detect both IC and IE with very high precision and recall.

% \jinqiu{This sounds an inheritated problem with micro clones? I don't think it is ``hard to identify'', as some tools are aimed at micro clones and claim good results. Can we say micro clone is an on-going research effort and partially remain subjective, and are less likely caused by maintenance debt? We can find some insights from that SANER 2019 paper.}
%\zhenhao{Don't know how to connect with Micro-clones, since they define micro-clones as clones that no more than five lines of code, however our threshold is 10.}\peter{just add the citation somewhere, we don't need to discuss in detail} \zhenhao{Discussed about it in related works.}

\noindent{\bf {\em LM: }}{\em 83\% of the LM instances are labeled as either Clones or Micro-clones.} As shown in Table~\ref{table:manualrq5}, 7 out of 30 instances are labeled as {\em Clones}, 18 out of 30 instances are labeled as {\em Micro-clones}, and the remaining 5 instances are labeled as {\em Non-clones}. For the five instances that are identified as {\em Clones}, they all belong to Category 2 (i.e., they share highly similar semantics, but have minor differences). The reason might be that developers copy and paste a piece of code along with the logging statement to another location, and apply some modifications to the code. However, developers forgot to change the log message. Similarly, for the five instances that are labeled as {\em Non-clones}, we find that even though the code is syntactically different, the log messages do not reflect the associated method. For the 18 {\em Micro-clones} instances, 11 out of 18 instances belong to Category 3 (short methods), and the remaining 7 are Category 2 (short code snippets within a larger code block). As confirmed by the developers (in Section~\ref{sec:manual}), these LM instances are related to logging statements being copied from other places in the code without the needed modification (e.g., updating the method name in the log).

Our manual analysis on LM instances provides insights on possible maintenance problems that are related to the modification and evolution of cloned code. Future studies may further investigate the inconsistencies in the source code and other software artifacts (e.g., logs or comments) that are caused by code clone evolution.


%In our manual analysis, we find that the log messages indeed do not reflect the associated method (which is also confirmed by developers, as discussed in Section~\ref{sec:manual}). However, these logging statements are inside short methods or blocks, which make them difficult to detect using clone detection techniques.


%As confirmed by the developers, these logging statements are copied from other places in the code without the needed modification (e.g., to update the method name that is recorded in the log). Our finding provides insights on possible maintenance problems that are related to the modification and evolution of cloned code. Future studies may further investigate the inconsistencies in the source code and other software artifacts that are caused by code clone evolution. % and out-of-sync %software artchitecure (e.g., comments or logging statements).


%caused by the evolution and maintenance of cloned code snippets. Future studies may further investigate the inconsistencies that are caused by

%~\jinqiu{``This inspires futhure research might pay attention to the inconsistencies caused by clone evolution and out-of-sync semantic information such as logging statements."}

%developers modified the code significantly~\jinqiu{not sure about this, how do you find that it is due to copy and paste and then the code significantly?}, but they forgot to change the log messages. Therefore, even though the code is not considered clone, we still find inconsistent log messages. ~\jinqiu{``This inspires futhure research might pay attention to the inconsistencies caused by clone evolution and out-of-sync semantic information such as logging statements."}


%\peter{maybe remove this part}Compared to clone detection techniques, \toolS detects LM by analyzing log messages and the corresponding method names. Hence, \toolS may complement clone detection tools on finding LM instances~\jinqiu{how does clone detection tool find LM instances? If by firstly finding clond snippets, isn't that super inaccurate?} that are located in short code blocks.


%Similar to our observation for Clones, the reason might be that developers forget to consistently update the log message  when other code changes. Even though the code in short methods and short blocks might be generic, they are very likely caused by copy-and-paste (since their log messages does not match with the execution behavior), it is difficult to make a decision whether they are clones or intentionally written by developers (they might write the log messages improperly).

\noindent{\bf {\em DP: }}{\em 59\% of the DP instances are either Clones or Micro-clones, which may show that developers often copy code along with the logging statements across sibling classes.} In total, 32 out of 95 DP instances are labeled as {\em Clones}, 23 are labeled as {\em Micro-clones}, and the remaining 43 instances are labeled as {\em Non-clones}. For the 32 instances that are labeled as {\em Clones}, 16 instances are Category 1 (part of a large code block), the remaining 16 instances are Category 2 (very similar semantics with minor differences). For the 24 {\em Micro-clones} instances, 11 instances belong to Category 3 (short methods), and the remaining 13 are categorized as Category 1 (short code snippets within a larger code block).
%Combined with the results from the clone detection tool, around 70\%$\sim$81\% (\peter{the sentence in the bracket is not clear}144/207~\jinqiu{Where is this 207 from?} without any instances of Undecidable, 167/207 with all the instances of Undecidable \zhenhao{(112+32)=144 Clones, with 24 Undecidable instances out of 207 total instances. If 0 Undecidable instance is considered, then 70\%. If all, then 81\%. }) of the DP instances are related to code clones.
Combined with the results from the clone detection tool, around 81.2\% (112 detected by the tool + 32 Clones + 24 Micro-clones identified by manual study, out of 207 total instances) of the DP instances are related to code clones.
One possible reason of a higher percentage of DP instances being related to code clone is that DP is related to inheritance. Classes that inherit from the same parent class may share certain implementation details. Nevertheless, due to the similarity of the code, developers should consider updating the log messages to distinguish the executed methods during production to assist debugging runtime errors.

%However, as discussed in Section~\ref{sec:manual}, resolving DP often requires systematic refactoring, and the fixes of DP instances are not definitely expected as the technical debts need to be considered~\cite{Kruchten:2012:TDM:2412381.2412847}. \zhenhao{what can we learn from the view of code clones?}

%\jinqiu{I am forming one possible highlight here, not necessarily a correct argument: Our finding indicates that semantic information such as duplicate logging statements may serve as trails to distill copy-and-paste clones from general clones, which are commonly considered as bad programming practices and a source of bugs.}

%In summary, our finding indicates that the semantic information in the code, such as logging statements, may be used as trails to help


%\rqbox{Take-home box. \zhenhao{Todo: Talk about sth like LM instances usually locate in short blocks (shorter than 10 lines), so it might be hard for the existing clone detection approaches to find this kind of problems at the meantime of addressing code clone problems. More specific approaches or tools are needed to tackle it.}
%\zhenhao{Still a large portion of problematic instances reside in short methods / short blocks, current clone detection tools might not be able to detect them effectively.}\peter{@Zhenhao, see if you can come up with the takehome based on the updated discussions}
%}
\vspace{-0.1cm}
\rqboxc{We find that most of the instances of the problematic duplicate logging code smells (83.0\%, 240 out of 289 instances, combining the results of tool detection and manual study) are related to code clones. Our finding further shows the negative effect of code clones on system maintenance. Moreover, most problematic instances reside in short code blocks which might be difficult to detect by using existing code clone detection tools.
%Our findings may also highlight the potential of using duplicate logging statements to further improve clone detection tools.
}
\vspace{1mm}
\noindent{\bf Discussion: the potential of whether code clone detection tool can substitute or complement \tool.} As we discussed previously, most of the problematic instances of duplicate logging code smells (83.0\%) are related to code clones. We then discuss the potential of whether code clone detection tool can substitute or complement \toolS in terms of detecting problematic instances of duplicate logging code smells. We use the results of our code clone analysis as a baseline to compare with the detection results of \tool. Similar to our evaluation in Section~\ref{sec:results}, we only compare the detection results of LM since the other patterns are well-defined and relatively independent of the surrounding code. LM depends on the semantics of the logging statement and its surrounding code, of which the detection might potentially be helped by code clone analysis. We consider the code clones that contain duplicate logging statements as the total amount of detected instances. We then analyze the clone detection results and match the location of the clones with that of the ground truth instances of LM. If two or more cloned code snippets contain the logging statements of an LM instance, we consider the duplicate logging statements of this instance as a true positive. Overall, the average precision and recall of this baseline in the manually studied systems are 3.7\% and 53.7\%, respestively. The average precision and recall in the additional systems are 1.5\% and 38.9\%, respectively. In terms of the performance of detection, our approach is noticeably better than this baseline. Moreover, as we discussed in Section~\ref{sec:results}, 10 out of 59 instances of LM are not detected by \tool. Among them, 4 out of 10 instances are detected by this baseline approach. We investigate those instances and find those log messages and class method names are at different levels of abstraction: The log message describes a local code block while the class-method name describes the functionality of the entire method (similar to what we discussed in Section~\ref{sec:results}). In this kind of scenarios, the code clone analysis outperforms our detection rule, which might be an inspiration of improving our detection rule. But it still remains a complicated task for us to balance the trade-off of a few more true positives and much more false positives for merging the code clone analysis into our detection approach. In short, although most of the problematic instances of duplicate logging code smells are related to code clones, they can not be effectively detected by clone detection tools.
%RQ1 systems: GT: 37, TP:20, Detected: 498, for 4+4
%RQ2 systems: GT: 22, TP: 9, Detected: 544, for 4+4
%10 instaces missed by DLFinder
\vspace{-0.1cm}

\noindent{\bf Implication and highlights of our code clone analysis.} Our finding shows that most of duplicate logging statements are indeed related to code clones (i.e., regular clones and micro-clones), and many of which cannot be easily detected by state-of-the-art clone detection tools. Our finding shows additional maintenance challenges that may be introduced by code clones -- understanding the runtime behaviour of system execution. We find that duplicate logging statements may also be a possible indication of hard-to-detect clones based on our manual study. Moreover, most of the problematic instances of duplicate logging code smell reside in cloned code snippets. Hence, future code clone detection studies should consider other possible side effects of code clones (e.g., understanding system runtime behaviour) in addition to code maintenance and refactoring overheads. Future studies may also consider integrating different information in the software artifacts (e.g., duplicate logging statements or comments) to further improve clone detection results. %when implementing clone detection tools. %that for the code snippets that are not detected as clones





\begin{comment}

\begin{table*}
  \caption{The result of manual study in Secion~\ref{sec:clone} {\sf DupSet}: Sampled sets of duplicate logging statements, discussed in RQ4. {\sf IC, IE, LM, DP}: Instances of each pattern, discussed in RQ5.\peter{let's break the Table into 2. Otherwise, in RQ5, we need to keep look at Table 7 which is far away from the discussion}\jinqiu{Missing the category of Non-cloned}}
    \vspace{-0.3cm}
    \centering
    %\resizebox{\textwidth}{!} {
    \tabcolsep=8pt
    \scalebox{0.8}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}

        \toprule
     & \multicolumn{3}{c|}{\textbf{DupSet}} & \multicolumn{3}{c|}{\textbf{IC}} & \multicolumn{3}{c|}{\textbf{IE}} & \multicolumn{3}{c|}{\textbf{LM}} & \multicolumn{3}{c}{\textbf{DP}} \\
     &Clones &Undec. & Total &Clones &Undec. & Total &Clones &Undec. & Total &Clones &Undec. & Total &Clones &Undec. & Total \\
\midrule

        \textbf{Cassandra}    & 1 & 3 & 7    & 0 & 0 & 1     & 0  &0  & 0     & 0 & 0 & 0     &  0  &0 &0 \\
        \textbf{CloudStack}    & 22 & 26 & 94    & 0  &3 & 3    & 0 &0 & 0    & 1  &5 & 7     & 12 &9 &47 \\
        \textbf{ElasticSearch} & 1 & 1 & 5    & 0 & 0 & 1      & 0 &0  & 0   &0  &1  & 1       & 1  &0  &3\\
        \textbf{Hadoop}      & 12 & 6 & 43    & 0  &2 & 4     & 0 &0  & 0   &3  &3  & 9       & 14  &6  &22\\

       \textbf{Camel}       & 28 & 30 & 103    & 0 &1 & 1     & 0  &0 & 0    & 2 & 6 & 8      &2 &4  &7\\
       \textbf{Flink}       & 5 & 4 & 25    & 0 &0 & 0     & 0 &1 & 1    & 0 & 2 & 2       &0  & 3 &5\\
       \textbf{Kafka}       & 3 & 7 & 18    & 0  &0 & 0    & 0 &0 &0    & 0  &1  &2     & 3 & 2 &11 \\
       \textbf{Wicket}       & 1 & 1 & 3    & 0 &0 & 1       & 0 &0 & 0     & 1 &0  &1          & 0 &0  &0 \\

        \midrule

        \textbf{Total}       & 73 &78 & 298     & 0 &6 & 11    & 0 &0  &1     & 7 & 18 &30         &32 &24 &95\\


        % cass non-dup median 7, 0.146 neg
        % cloud stack non-dup median 8, 0.045 neg
        % es non-dup median 7, 0.27 small
        % hadoop non-dup median 6, 0.08 neg
        \bottomrule
    \end{tabular}}
    %}
    \vspace{-0.3cm}

    \label{table:manualrq5}
\end{table*}

\end{comment}


==> texfiles/backup/manual_old.tex <==
\section{Manually Characterizing Duplicate Logs}
\label{sec:manual}

%\peter{might need to change the motivation based on the new intro}Similar to duplicate code or code clones, having duplicate logs may or may not be a problem~\cite{kapser2006a}. 

In this section, we manually study and characterize duplicate logs with two goals. First, we study duplicate logs and the surrounding code to understand whether duplicate logs are associated to code clones. Also, we manually uncover patterns of duplicate logging code smells that may be an indication of problems and require refactoring. The uncovered patterns of duplicate logging code smells will be utilized in a semi-automated approach to detect more instances of duplicate logging code smell at a large scale in Section~\ref{sec:userstudy}.
Figure~\ref{fig:overall} illustrates the overall process of our study. 

 \begin{figure*}
 \centering
\includegraphics[width=0.85\linewidth]{figures/overallShorten.pdf}
\vspace{-0.3cm}
 \caption{The overall process of our study.}
 \vspace{-0.3cm}
 \label{fig:overall}
 \end{figure*}


% <<<<<<< HEAD
% In this section, we manually study duplicate logs and the surrounding code to understand potential causes (e.g., are they caused by code clones). We also manually uncover patterns of duplicate logging code smells that may be an indication of problems and require refactoring. Figure~\ref{fig:overall} illustrates the overall process of our study. 


% \subsection{Manually Studying Duplicate Logs}

% \phead{Motivation.}
% We have two goals in our manual study. Our first goal is to study whether such duplicate logs are caused by developers copying and pasting the log statements and their surrounding code to different places (i.e., code clones). 
% Prior code clone studies focus on finding whether two pieces of code are syntactically or semantically similar~\cite{roy09}. 
% Although prior code clone studies do not specifically target duplicate logs, one may wonder if duplicate logs reside in cloned code.
% %However, one may wonder if the log messages are the same in two methods, would the code in these two methods be clones of each other. 
% Hence, we want to investigate how many duplicate log sets are in cloned code. A potential way of identifying code clones is to use tools such as CCFinder~\cite{kamiya2002}, but clone detection techniques usually requires setting a certain thresholds~\cite{roy09}. Non-optimal thresholds have significant impacts on the detected clones~\cite{roy09, 7081830}. However, choosing the optimal thresholds is a non-trivial task and the value may differ across systems~
% \cite{nikos_icse_2018}. Therefore, instead of running automated clone detection tools, the first two authors of the paper manually examine the sampled duplicate logs and the surrounding code, to study whether the duplicate logs are related to code clones. 
% =======
\subsection{Manually Studying Duplicate Logs}

\phead{Motivation.}
We have two goals in our manual study. Our first goal is to study whether there is a relationship between duplicate logs and code clones. For example, duplicate logs may be caused by developers copying and pasting the log statements and their surrounding code to different places (i.e., code clones). 
%Prior code clone studies focus on finding whether two pieces of code are syntactically or semantically similar~\cite{roy09}. 
Although prior code clone studies do not specifically target duplicate logs, one may wonder if duplicate logs reside in cloned code.
Hence, we want to investigate how many duplicate log sets are associated with cloned code. A potential way of identifying code clones is to use tools such as CCFinder~\cite{kamiya2002}, but clone detection techniques typically require setting a certain thresholds~\cite{roy09}. Non-optimal thresholds have significant impacts on the detected clones~\cite{roy09, 7081830}. However, choosing the optimal thresholds is a non-trivial task and the value may differ across systems~
\cite{nikos_icse_2018}. 
%\jinqiu{From here to the end of the paragraph, should go to `Approach'}
Therefore, instead of running automated clone detection tools, the first two authors of the paper independently examine the sampled duplicate logs and the surrounding code, to study whether the duplicate logs are related to code clones. 
%>>>>>>> f838390c4a22eb66c321e45065b34eac772fdb4f

Our second goal is to identify duplicate logging code smells. Similar to prior code smell studies~\cite{budgen2003software, fowler1999refactoring}, we define duplicate logging code smells as a {\em ``surface indication that usually corresponds to a deeper problem in the system''}. Most current log-related research focuses on identifying ``where to log''~\cite{Yuan:2010:SED:1736020.1736038, Zhu:2015:LLH:2818754.2818807, kundi_icpe_2018} and ``what to log''~\cite{Yuan:2011:ISD:1950365.1950369, Shang:2014:ULL:2705615.2706065}. Nevertheless, knowing how to help developers refactor logging code and provide the needed supports can help improve various tasks such as debugging and testing~\cite{Shang:2014:ULL:2705615.2706065, Chen:2017:ALT:3103112.3103144}. %Similar to code clones, duplicate logs may or may not be a problem~\cite{kapser2006a}. 
Therefore, we want to manually study duplicate logs and uncover patterns of duplicate logging code smells that may be indications of logging problems that require log refactoring. Since some duplicate logs may not be a problem, uncovering code patterns of duplicate logging code smells help us narrow down the problems and conduct further detailed analysis.% on duplicate logging code smells. 



\phead{Approach.}
%To study the causes of the duplicate logs (e.g., code clone or the logs are the same by coincident), 
We conduct a manual study by randomly sampling a total of 289 sets of duplicate logs (based on 95\% confidence level and 5\% confidence interval~\cite{boslaugh2008statistics}). Since the number of duplicate logs vary significantly across the studied systems, similar to prior studies~\cite{log_pattern_ICSE2017, boslaugh2008statistics}, we use the stratified sampling technique. We calculate the sample size according to the number of duplicate logs in each studied system. As an example, we detected a total of 1,168 sets of duplicate logs (i.e., each set contains two or more logs with the same message) in all the studied systems, and 865 of them are in CloudStack (74\%). Therefore, we sample $74\% * 289 = 213$ sets of duplicate logs from CloudStack. Similarly, we detected 217, 46, and 40 sets from Hadoop, Cassandra, and ElasticSearch, and we sampled 54, 12, and 10 sets, respectively. To uncover patterns of duplicate logging code smells, \peter{explain open coding, how many iteration, describe merger and split}we follow a lightweight open coding-like process to identify the patterns in which the duplicate log belongs~\cite{seaman1999qualitative}. Namely, we first go through the sets of duplicate logs to uncover possible code patterns. %Our first goal is to manually derive the categories of the causes. 
Then, we go through the duplicate logs again and assign them to the corresponding pattern. 

%, where 46 are in Cassandra, 864 are in CloudStack, 217 are in Hadoop, and 40 are in ElasticSearch. Based %Logs are stored as Map structure of which key is the syntactic message, value is a set of all the call-sites of this logging statement. 

%As an example,\zhenhao{We detected totally 1171 sets of duplicate logs in our subject systems, 218 sets were detected from Hadoop which accounts for 18.6\% of the total sets. Thus we will manually study 54 sets in Hadoop.} \zhenhao{ Accordingly, we detected 47, 865, and 41 sets from Cassandra, Cloudstack, and Elasticsearch respectively. Therefore we will sample 12, 213, and 10 sets from each system.} \peter{TODO: Zhenhao, can you fill in the numbers?}\peter{TODO: Zhenhao, add an example on how we calculate this}. \peter{TODO: Zhenhao, say how many we selected from each system} 



\subsection{Studying the Relationship Between Duplicate Logs and Code Clones}%~\jinqiu{Are duplicate logs caused by code clones? or others, it is not clear this section shows results from the title, so is the title of next section} 

% \peter{prior code clones study do not consider log clones (log message or other string constant). One may wonder if they are related }\peter{need to mention they are exact copy or part of the code is exact copy with small modification}
\phead{{\em We find that 40\% of the duplicate logs are not related to code clones.}} We find that, among all the manually studied duplicate logs, 60\% are related to code clone (vary between 59\% to 73\% for the studied systems), whereas 40\% are not related to code clone. We identify if the surrounding code of two duplicate logs is clone if we see syntactic similarities. We use Cohen's kappa~\cite{kappa} to measure the inter-rater agreement between the first two authors of the paper. Any disagreement is discussed until a consensus is reached. %, we discuss until an agreement is reached. 
The value of Cohen's kappa is above 0.9 for all studied systems (i.e., a high-level of agreement~\cite{kappa}). Our finding shows that, although many duplicate logs are related to code clones, there is still a significant number of duplicate logs that are not related to code clones. %related to the methods having similar log messages but different code structure.%~\jinqiu{I don't understand what are `methods having similar log messages'. Revisit} 
\todo{improve the manual}

%\peter{Zhenhao, maybe discuss how many dup logs which are not caused by clones are generic logs/too short logs. We can easily get those logs from the google sheet, and then we only need to count number of words in each group} \zhenhao{For duplicate logs which are not caused by code clone, we find that 16\% (18/111) of them are generic or too short logs}\peter{it is hard to explain what is generic or what is too short. report the number of words is better} \todo{Zhenhao, can you get the new number for me here (mean and median for each system, either C or NC)? I remember you have it in the slide} \zhenhao{Updated those numbers in the comment below. Those short logs were not filtered, can we double-check all the numbers after the first draft, and shape all of them with the same regulation? So far some number are filtered with length<1, some are 2, some are not...} 

% cassandra total 15, 4 not clone (31%), clone is 11 (73%) avg(C): 14.2, avg(NC): 4.3, med(C):14, med(NC):2.5 
% elastic search total 10, 4 not clone (40%), clone is 6 (60%) avg(C):7, avg(NC):4, med(C):5.5, med(NC):3.5
% hadoop total 40, 15 not clone (37.5%), clone is 25 (62.5%) avg(C): 8.2, avg(NC): 5.2, med(C): 8, med(NC):4
% cloud stack total 213, 88 not clone (41%), clone is 125 (59%) avg(C): 11.2, avg(NC):7, med(C):10, med(NC):6
% total 278, total not clone 111, total clone 167
% Those short logs were not filtered, can we double-check all the numbers after the first draft, and shape all of them with the same regulation? 


% \begin{table*}
% \caption{Patterns of duplicate logging code smells 
% and corresponding examples.} %\ahmed{nothing about parallel development or is that showing up as a theme throughout the different challenges?}
% \centering
% %\resizebox{\textwidth}{!} {%
% %\begin{adjustbox}{width=1\textwidth}

% \begin{tabular}{ m{2.5cm}|l}
% \toprule
% \textbf{Name} & \textbf{Example} \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
% %This example is from Cloudstack, com.cloud.api.dispatch.ParamProcessWorker.processParameters
% Inadequate information in catch blocks (IC) & \begin{lstlisting}
% /* log message cannot be used to distinguish which exception occurred */
% catch (final IllegalArgumentException e) {
%     s_logger.error("Error initializing command " + cmd.getCommandName() 
%      + ", field " + field.getName() + " is not accessible.");
%     ... 
% } catch (final IllegalAccessException e) {
%     s_logger.error("Error initializing command " + cmd.getCommandName() 
%      + ", field " + field.getName() + " is not accessible.");
%     ... 
% }
% \end{lstlisting}\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
% %This example is from Cloudstack
% Inconsistent error diagnostic information ({\sf IE}) & \begin{lstlisting}
% public class CreatePortForwardingRuleCmd{
%     ...
%     } catch (NetworkRuleConflictException ex) {
%     s_logger.info("Network rule conflict: " + ex.getMessage());
%     ...
% }
% ------------------------------------------------------------------------
% public class CreateFirewallRuleCmd{
%     ...
%     } catch (NetworkRuleConflictException ex) {
%     s_logger.info("Network rule conflict: ", ex);
%     ...
% }
% \end{lstlisting}\\

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
% %This example is from Hadoop
% Duplicate log in inheritance ({\sf DI}) & \begin{lstlisting}
% public class PowerShellFencer extends Configured implements FenceMethod {
%     ... /* class-specific implementation for FenceMethod */
%     } catch (InterruptedException ie) {
%       LOG.warn("Interrupted while waiting for fencing command: " + ps1script);
%     ...
% }
% ------------------------------------------------------------------------
% public class ShellCommandFencer extends Configured implements FenceMethod {
%     ... /* class-specific implementation for FenceMethod */
%     } catch (InterruptedException ie) {
%       LOG.warn("Interrupted while waiting for fencing command: " + cmd);
%     ...
% } 
% \end{lstlisting}\\

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
% %This is from Cassandra, same class: CompactionManager 
% Inconsistent log level ({\sf L}) & \begin{lstlisting}
% /* log levels are different in two very similar methods */
% public AllSSTableOpStatus performCleanup(){
%     ...
%     if (!StorageService.instance.isJoined()){
%         logger.info("Cleanup cannot run before a node has joined the ring");
%         return AllSSTableOpStatus.ABORTED;
%     }
%     ...
% }
% ------------------------------------------------------------------------
% public void forceUserDefinedCleanup(){
%     ...
%     if (!StorageService.instance.isJoined()){
%         logger.error("Cleanup cannot run before a node has joined the ring");
%         return;
%     }
%     ...
% }            
% \end{lstlisting}\\

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
% %This is from CloudStack
% Log message mismatch ({\sf M}) & \begin{lstlisting}
% public void doScaleUp() {
%     ...
%     s_logger.error("Can not find the groupid " + groupId + " for scaling up");
%     ...
% }
% ------------------------------------------------------------------------
% public void doScaleDown() {
%     ...
%     /* a copy-and-paste error; scaling up is the behavior of the above-mentioned method */
%     s_logger.error("Can not find the groupid " + groupId + " for scaling up");
%     ...
% }
% \end{lstlisting}\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \bottomrule
% \end{tabular}
% %}
% %\end{adjustbox}
% \label{tab:patterns}
% \end{table*}



\begin{table*}
\caption{Patterns of duplicate logging code smells 
and corresponding examples.} %\ahmed{nothing about parallel development or is that showing up as a theme throughout the different challenges?}
\centering
%\resizebox{\textwidth}{!} {%
%\begin{adjustbox}{width=1\textwidth}

\begin{tabular}{m{.2\textwidth} | m{.65\textwidth}  }%{ m{3cm} |l}
\toprule
\textbf{Name} & \textbf{Example} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%This example is from Cloudstack, com.cloud.api.dispatch.ParamProcessWorker.processParameters
Inadequate information in catch blocks (IC) & 
\includegraphics[width=0.65\textwidth]{figures/manual_IC}

\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%This example is from Cloudstack
Inconsistent error diagnostic information (IE) & \includegraphics[width=0.65\textwidth]{figures/manual_IE}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%This is from CloudStack
Log message mismatch (LM) & \includegraphics[width=0.65\textwidth]{figures/manual_M}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
%This is from Cassandra, same class: CompactionManager 
Inconsistent log level (IL) & \includegraphics[width=0.65\textwidth]{figures/manual_L}
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
%This example is from Hadoop
Duplicate log in polymorphism (DP) & \includegraphics[width=0.65\textwidth]{figures/manual_DI}
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bottomrule
\end{tabular}
%}
%\end{adjustbox}
\label{tab:patterns}
\end{table*}

\subsection{Manually Uncovering Patterns of Duplicate Logging Code Smells}
%In this subsection, we document the duplicate logging code smells that we uncovered during manual analysis. 
\phead{{\em In total, we uncovered five patterns of duplicate logging code smells.}} Table~\ref{tab:patterns} lists the uncovered patterns of duplicate logging code smells and the corresponding examples. Below, we describe each pattern in detail and discuss its potential problems. Note that these uncovered patterns are indications of potential problems. We use these patterns as a starting point to find more instances of duplicate logging code smells. In Section~\ref{sec:userstudy}, we further conduct a detailed manual analysis on the impact of each pattern by classifying each pattern into sub-categories (i.e., some sub-categories may require refactoring while others may not). 

%The uncovered patterns are our starting point to find more instances of duplicate logging code smells, and so that later we provide a more detailed analysis of impact on each pattern by classifying each pattern into sub-categories (i.e., some sub-categories require refactoring while others do not) in Section~\ref{sec:userstudy}.~\jinqiu{Please check this para.}

\phead{Inadequate information in catch blocks (IC).} Developers usually rely on logs for error diagnostics when exceptions occur~\cite{Yuan:2014:STP:2685048.2685068}. However, we find that sometimes, duplicate logs in the {\em catch} block of different exceptions may cause debugging difficulties since the logs fail to tell which exception occurred. As shown in Table~\ref{tab:patterns}, in the {\em ParamProcessWorker} class in CloudStack, the \em{try} block contains two {\em catch} blocks; however the log messages in these two {\em catch} blocks are identical. Since both the exception message and stack trace are not logged, once one of the two exceptions occurs, developers may encounter difficulties in finding the root causes and determining the occurred exception. %Therefore, developers should either add extra information (e.g., exception type or stack trace) to the log or change the log message to avoid debugging. %On the other hand, if the log messages are different or if the log records stack trace information, developers may use the recorded information to debug the occurred exception. %log messages may not contain sufficient information for developers to debug the occurred exception.  

\phead{Inconsistent error diagnostic information (IE).} We find that sometimes duplicate logs may contain inconsistent error diagnostic information. Namely, the recorded dynamic variables are different (e.g., one log records the stack trace but the other log does not), even though the surrounding code is very similar. As shown in Table~\ref{tab:patterns}, the two classes {\tt\small Create\textbf{PortForwarding}RuleCmd} and {\tt\small Create\textbf{Firewall}RuleCmd} in CloudStack have similar functionality. The two log statements have the same static text message and are in methods with identical names (i.e., {\em create()}, not shown due to space restriction). The two {\em create()} methods have very similar code structure and perform very similar functionalities. The {\em create()} method in {\tt\small Create\textbf{PortForwarding}RuleCmd} is about creating rules for port forwarding and the the method in {\tt\small Create\textbf{Firewall}RuleCmd} is about creating rules for firewalls. However, the two log statements record different information: One records the stack trace information and the other one only records the exception message (i.e., {\em ex.getMessage()}). Due to the similar context of the two log statements, the error diagnostic information that is recorded by the logs may also need to be consistent \peter{not sure if we need to mention this here: }(we reported this problem to developers and it is now fixed as we suggested). %should also be similar. 


%\todo{Zhenhao, can you describe the example? Like if they are very similar class and briefly what these two methods do. We want to argue that, these two methods are very similar, but developers still log differently} \zhenhao{CreatePortForwardingRUleCmd and CreateFirewallRuleCmd. Both of these two logging statements are included in methods create(). The upper example is about creating rule for port forwarding, the under one is about creating rule for firewall. These two logging statements have identical messages and code context, but one logs stack trace with a variable "ex" which was introduced by a developer 4 years ago, the other one just log the exception message "ex.getMessage()" which was introduced 7 years ago. It seems that developer copied it from CreatePortForwardingRuleCmd, and changed the logging statement to log the full stack trace, but didn't change the origin one.} \peter{are you sure about the copying part? If not, we can just not mention it} \zhenhao{Not 100\% sure, because there are many differences between those two methods, only the catch blocks are very very similar.}


%When logging the same message, we find that the logs may sometimes contain inconsistent error diagnostic information (i.e., stack trace). As shown in Table~\ref{tab:patterns}, \peter{TODO: describe the example}



\phead{Log message mismatch (LM).} We find that sometimes after developers copy and paste a piece of code, they may forget to change the log message. As an example, in Table~\ref{tab:patterns}, the method {\em doScaleDown()} is a clone of {\em doScaleUp()} with very similar code structure and minor syntactical differences. However, developers forgot to change the log message in {\em doScaleDown()}, after the code was copied from {\em doScaleUp()} (i.e., both log messages contain {\em scaling up}). The problem causes confusion when developers analyze the logs~\cite{es-issue-forM}. % in the log lines when


%\peter{Zhenhao: which methods are the examples from?} \todo{Zhenhao, can you finish describing the example here?}\zhenhao{The upper example is included in method tryFence(HAServiceTarget target, String argsStr), the under one is included in tryFence(HAServiceTarget target, String cmd). The functions of try statements which manage those catch clauses are identical, only with a difference of variables in the logging statements. The upper example attaches a variable "ps1script" to log message, the under one attaches "cmd" to the log messages, which is also the parameter of it's method. (What can we learn from this example?)}



\phead{Inconsistent log level (IL).} Log levels (e.g., {\em fatal}, {\em error}, {\em info}, {\em debug}, or {\em trace}) allow developers to specify the severity of the log message and to reduce logging overhead when needed (e.g., {\em debug} is usually disabled in production)~\cite{Li2017}. A prior study~\cite{Yuan:2012:CLP:2337223.2337236} shows that log level is frequently modified by developers in order to find the most adequate level. We find that there are duplicate logs that, even though the log messages are exactly the same, %\todo{Zhenhao, can you quickly get the number of words for these logs?} \zhenhao{Now it have the med and avg words for them, should I filter those short ones? and how short should I filter?}\peter{maybe filter out those with only 2 words} \zhenhao{I find that some 2-length ones are meaningful, so for this time I filtered those shorter than 1. The numbers are in the comment below}, 
the log levels are different. 
%We also find that such duplicate logs with inconsistent levels are often {\em not} generic logs (i.e., median length of duplicate logs with inconsistent levels is 6 words). The log message in generic logs could be identical by chance, thus inconsistent log level in generic logs maybe by intent~\jinqiu{Check please.}.%where the log levels might be different by chance. 
As shown in Table~\ref{tab:patterns}, the two methods are both from the class ({\tt\small CompactionManager}) in Cassandra. The two methods have very similar functionality (i.e., both try to perform cleanup after compaction), but we find that the log levels are different in these two methods. %\todo{Zhenhao, for this particular example, was it copied from one method?} \zhenhao{No, look like it's not. The context are so different }
% Link to the L example: https://github.com/apache/cassandra/blob/trunk/src/java/org/apache/cassandra/db/compaction/CompactionManager.java
%avg length of data set in L: 6.6,   med: 6


\phead{Duplicate log in polymorphism (DP).} Classes in object-oriented languages are expected to share similar functionality if they inherent the same parent class or if they implement the same interface (i.e., polymorphism). Since log messages record a higher level abstraction of the program~\cite{Shang:2014:ULL:2705615.2706065}, we find that even though there are no clones among a parent method and its overridden methods, such methods may still contain duplicate logs. %, which have similar functionalities,%the log messages may be the 
% the code in the inherited methods may not necessarily be clone, but the log messages may be the same due to the methods having similar functionalities. 
%Due to the similarity, we find that developers may put the same log messages in the sibling classes or in the parent class. 
%\peter{log message record a higher level abstraction of the log. in the particular situation of DI, the code may not necessarily clone, but the log message should be similar. This opens a door for refactoring}
Such duplicate logs may cause maintenance overhead. For example, when developers update one log message, he/she may forget to update the log message in all the other sibling classes. Inconsistent log messages may cause problems during log analysis~\cite{mehran_emse_2018, HADOOP-4190}. %or may even cause incorrect test analysis results\peter{some citations?}. 
As shown in Table~\ref{tab:patterns}, the two classes ({\tt\small PowerShellFencer} and {\tt\small ShellCommandFencer}) in Hadoop share similar behaviours, and both classes extend the same parent class and implement the same interface. The log lines in both classes have the identical message in the inherited method. However, as systems evolve, developers may not always remember to change the log lines in both methods, which may cause problems during system debugging, understanding, and analysis.  

\hypobox{We find that 40\% of the duplicate logs are not related to code clones. We also uncover five patterns of duplicate logging code smells based on our manual study on a statistical sample of duplicate logs.}

\begin{comment}
\subsubsection{Duplicate Log Patterns} 
\peter{for the patterns of duplicate logs, each of them, we should say, whether logging library should have some new mechanism to support these patterns, instead of developers use duplicate logs to hack these.}
Below, we discuss three general duplicate log patterns we observe that are added intentionally by developers. \peter{I only have two right now, can you think of another one, or you think two is enough?}

%https://github.com/apache/hadoop/blob/f67237cbe7bc48a1b9088e990800b37529f1db2a/hadoop-common-project/hadoop-common/src/main/java/org/apache/hadoop/ipc/Client.java


\phead{Inconsistent log levels in different control flow ({\tt IC}).} 
\peter{maybe see which one makes more sense}
\zhenhao{all of them make sense I think, maybe the third one is better?}
\begin{lstlisting}
if (currRetries < maxRetries) {
    if(LOG.isDebugEnabled()) {
        LOG.debug("Exception encountered while connecting to "
                    + "the server : " + ex);
    }
    ...
} else {
    LOG.warn("Exception encountered while connecting to "
                + "the server : " + ex);
}              
\end{lstlisting}

\begin{lstlisting}
if (e instanceof ClusterBlockException) {
    if (logger.isTraceEnabled()) {
        logger.trace("Failed to execute IndicesStatsAction for ClusterInfoUpdateJob", e);
    }
} else {
        logger.warn("Failed to execute IndicesStatsAction for ClusterInfoUpdateJob", e);
}
\end{lstlisting}

\begin{lstlisting}
switch (threshold) {
    case WARN:
        if (logger.isWarnEnabled()) 
            logger.warn(SLOW_GC_LOG_MESSAGE, ...);
            break;
    case INFO:
        if (logger.isInfoEnabled())
            logger.info(SLOW_GC_LOG_MESSAGE, ...);
            break;
     ...
}
\end{lstlisting}

\phead{Duplicate logs in inheritance ({\tt DI}).} We find that there may exist duplicate logs in classes that share the same superclass. Listing~\ref{code:di} shows an example of {\tt DI} in CloudStack. We observe that since developers often provide similar log messages to the same children classes, sometimes there may exist duplicate logs. \peter{may need to improve this}Moreover, due to the differences in the implementation, information such as log levels may also differ. For example, in {\tt NfsSecondaryStorageResource}, the operation can only happen inside service VM (as indicated by the developer's comment), so the log level is set to {\tt warn}. On the other hand, the same log message is set to {\tt info} in {\tt ConsoleProxyResource}.  %, and such duplicate logs may even have  
%com.cloud.agent.resource.consoleproxy.ConsoleProxyResource.configure,org.apache.cloudstack.storage.resource.NfsSecondaryStorageResource.configure
\begin{lstlisting}[caption={An example of duplicate log pattern in inheritance ({\tt DI}) in CloudStack.} \label{code:di}]
public class ConsoleProxyResource extends ServerResourceBase{
    ...
	@Override
    public boolean configure(String name, Map<String, Object> params) throws ConfigurationException {
        _localgw = (String)params.get("localgw");
        _eth1mask = (String)params.get("eth1mask");
        _eth1ip = (String)params.get("eth1ip");
        if (_eth1ip != null) {
            params.put("private.network.device", "eth1");
        } else {
            s_logger.info("eth1ip parameter has not been configured, assuming that we are not inside a system vm");
        } 
        .../* class-specific implementation */
    }
}

public class NfsSecondaryStorageResource extends ServerResourceBase{
    ...
	@Override
    public boolean configure(String name, Map<String, Object> params) throws ConfigurationException {
        _eth1ip = (String)params.get("eth1ip");
        _eth1mask = (String)params.get("eth1mask");
        if (_eth1ip != null) { // can only happen inside service vm
            params.put("private.network.device", "eth1");
        } else {
            s_logger.warn("eth1ip parameter has not been configured, assuming that we are not inside a system vm");
        }
        .../* class-specific implementation */
    }
}   

\end{lstlisting}


%https://github.com/apache/hadoop/blob/6ba9587d370fbf39c129c08c00ebbb894ccc1389/hadoop-hdfs-project/hadoop-hdfs/src/main/java/org/apache/hadoop/hdfs/server/datanode/fsdataset/ReplicaInputStreams.java
% Could not get file descriptor for inputstream of class

\subsubsection{Duplicate Log Anti-patterns}
During our manual study process, we also observe a number of anti-patterns that are associated with duplicate logs. Such anti-patterns may be an indicator of a logging problem. Below, we document three duplicate log anti-patterns that we observed.

\phead{Log message mismatches ({\tt M}).} We find that developers may forget to change the class/method name in the log message after copying the code to another place. As shown in Listing~\ref{code:m}, the correct log message in {\tt tryVirtualLock()} should be ``{\em cannot virtual lock because...}''. However, because the code was copied from {\tt tryMlockall()}, the message was incorrect. The problem was detected by our anti-pattern detector (Section~\ref{sec:detection}) and was reported and fixed by ElasticSearch developers~\cite{elasticsearch_m}. 

\begin{lstlisting}[caption={An example of log message mismatch anti-pattern ({\tt M}) in ElasticSearch. The problem was reported and fixed~\cite{elasticsearch_m}.} \label{code:m}]
static void tryMlockall() {
    if (!JNA_AVAILABLE) {
        logger.warn("cannot mlockall because JNA is not available");
        return;
    }
    JNANatives.tryMlockall();
}

static void tryVirtualLock() {
    if (!JNA_AVAILABLE) { /* a copy-and-paste error */
        logger.warn("cannot mlockall because JNA is not available");
        return;
    }
    JNANatives.tryVirtualLock();
}
\end{lstlisting}


\phead{Inconsistent error diagnostician information ({\tt IE}).} 
\peter{need to find another example. This one might not be a problem}
\begin{lstlisting}[caption={Inconsistent error diagnostician information ({\tt IE}) in Cassandra.} \label{code:di}]
public class StreamReader{
...
	@Override
    public SSTableMultiWriter read(DataInputPlus inputPlus) throws IOException {
...
        catch (Throwable e)
        {
            Object partitionKey = deserializer != null ? deserializer.partitionKey() : "";
            logger.warn("[Stream {}] Error while reading partition {} from stream on ks='{}' and table='{}'.",
                        session.planId(), partitionKey, cfs.keyspace.getName(), cfs.getTableName(), e);
            if (writer != null)
            {
                writer.abort(e);
            }
            throw Throwables.propagate(e);
        }
    }
...    
}

public class CompressedStreamReader extends StreamReader{
...

     public void rewriteOVFFile(final String origOvfFilePath, final String newOvfFilePath, final String diskName) {
...
catch (Throwable e)
        {
            Object partitionKey = deserializer != null ? deserializer.partitionKey() : "";
            logger.warn("[Stream {}] Error while reading partition {} from stream on ks='{}' and table='{}'.",
                        session.planId(), partitionKey, cfs.keyspace.getName(), cfs.getTableName());
            if (writer != null)
            {
                writer.abort(e);
            }
            if (extractIOExceptionCause(e).isPresent())
                throw e;
            throw Throwables.propagate(e);
        }
    }
...
}   

\end{lstlisting}

\phead{Inconsistent log level ({\tt L}).} \zhenhao{maybe L should not be considered as an anti-pattern} In some cases, we find that two logs in very similar code may have different log level. As shown in Listing~\ref{code:l}, the two methods are clones of each other (Type II clone), but the log levels are inconsistent (one is error and one is debug).  

\begin{lstlisting}[caption={An example of inconsistent log level anti-pattern ({\tt L}) in CloudStack.} \label{code:l}]
actually, I think this is not a problem...need to find anther example
public class SimulatorInvestigator extends AdapterBase{
    ...
    @Override
	public Status isAgentAlive(Host agent) {
    	... // code clone
    	catch (Exception e) {
        	s_logger.debug("Failed to send command to host: " + neighbor.getId()); /* debug log */
    	}
		...    
	}
	...
}

public class Ovm3Investigator extends AdapterBase{
	...
	@Override 
	public Status isAgentAlive(Host agent) {
    	... // code clone
    	catch (Exception e) {
            LOGGER.error("Failed to send command to host: " + neighbor.getId(), e); /* error log */
    	}
    	...
	}
	...
}
\end{lstlisting}



%We release our manual study result %For each individual studied system, the percentage of duplicate logs that are caused by clones vary between \peter{might need to count if those not caused by clones are shorter?}
\end{comment}









==> texfiles/backup/manual_old_August.tex <==
\section{Manually Studying Patterns of Duplicate Logging Code Smells}
\label{sec:manual}

%In this section, we manually uncover patterns of duplicate logging code smells that may be an indication of problems and require refactoring. 
%Figure~\ref{fig:overall} illustrates the overall process of our study. 

Our first goal of the manual study is to identify potential code smells that may be associated with duplicate logging statements (i.e., duplicate logging code smells). Similar to prior code smell studies~\cite{budgen2003software, fowler1999refactoring}, we define duplicate logging code smells as a {\em ``surface indication that usually corresponds to a deeper problem in the system''}. Such duplicate logging code smells that may be indications of logging problems that require refactoring. 

Our second goal is to manually identify potentially problematic (i.e., require refactoring) or justifiable (i.e., do not require refactoring) cases of duplicate logging code smells, by understanding the surrounding code. Intuitively, one needs to consider the code context to decide whether a code smell instance is problematic and requires refactoring. As shown in prior studies~\cite{Zhu:2015:LLH:2818754.2818807, Fu:2014:DLE:2591062.2591175, Li2018}, logging decisions, such as log messages and log levels, are often associated with the structure and semantic of the surrounding code. Hence, in addition to identifying patterns of the duplicate logging code smells, we also manually categorize the code smell instances as potentially problematic (i.e., require refactoring) or justifiable (i.e., do not require refactoring). We believe that by providing a more detailed understanding of code smells (i.e., by studying the surrounding code), we may better assist developers with log refactoring and inspire future research.


%Since some duplicate logs may not be a problem, our goal is to manually uncover patterns of duplicate logging code smells that may be indications of logging problems that require refactoring.



\peter{I feel this entire paragraph can be removed, since they are repeating the intro}Most current log-related research focuses on identifying ``where to log''~\cite{Yuan:2010:SED:1736020.1736038, Zhu:2015:LLH:2818754.2818807, kundi_icpe_2018} and ``what to log''~\cite{Yuan:2011:ISD:1950365.1950369, Shang:2014:ULL:2705615.2706065}. Nevertheless, knowing how to help developers refactor logging code and provide the needed supports can help improve various tasks such as debugging and testing~\cite{Shang:2014:ULL:2705615.2706065, Chen:2017:ALT:3103112.3103144,Lin:2016:LCB:2889160.2889232}. %Similar to code clones, duplicate logs may or may not be a problem~\cite{kapser2006a}. 
Therefore, we want to manually study duplicate logs and uncover patterns of duplicate logging code smells that may be indications of logging problems that require refactoring. Since some duplicate logs may not be a problem, uncovering code patterns of duplicate logging code smells help us narrow down the problems and conduct a further detailed analysis.
%The uncovered patterns of duplicate logging code smells will be utilized in a semi-automated approach to detect more instances of duplicate logging code smell at a large scale in Section~\ref{sec:userstudy}.

% on duplicate logging code smells. 

%\peter{log statement vs logging statement} \zhenhao{All are replaced by logging statement}

%We conduct a manual study by randomly sampling a total of 289 sets of duplicate logs (based on 95\% confidence level and 5\% confidence interval~\cite{boslaugh2008statistics}). Since the number of duplicate logs varies significantly across the studied systems, similar to prior studies~\cite{log_pattern_ICSE2017, boslaugh2008statistics}, we use the stratified sampling technique. We calculate the sample size according to the number of duplicate logs in each studied system. As an example, we detected a total of 1,168 sets of duplicate logs (i.e., each set contains two or more logs with the same message) in all the studied systems, and 865 of them are in CloudStack (74\%). Therefore, we sample $74\% * 289 = 213$ sets of duplicate logs from CloudStack. Similarly, we detected 217, 46, and 40 sets from Hadoop, Cassandra, and ElasticSearch, and we sampled 54, 12, and 10 sets, respectively. To uncover patterns of duplicate logging code smells, we follow a lightweight open coding-like process to identify the patterns in which the duplicate log belongs~\cite{seaman1999qualitative}. Namely, we first go through the sampled sets of duplicate logs to uncover possible code smell patterns. We iterate the process until no new patterns emerge. %Our first goal is to manually derive the categories of the causes. Then, we go through the duplicate logs again and assign them to the corresponding pattern. 


\begin{comment}
This process involves 3 phases and is performed by the first
two authors (i.e., A1–A2) in this paper:
• Phase I: A1 derived a draft list of types of performed
actions based on 50 random answers. Then, A1 and
A2 use the draft list to categorize the answers collaboratively. During this phase the types are revised and refined.
• Phase II: A1 and A2 independently applied the re-
sulting types from Phase I to categorize all 384 an-
swers. A1 & A2 took notes regarding the deficiency or ambiguity of the labeling for obsolete answers.
• Phase III: A1, A2 discussed the coding results that were obtained in Phase II to resolve any disagreements until a consensus was reached. No new types of labeling were added during this discussion. The inter-rater agreement of this coding process has a Cohen’s kappa of 0.97, which indicates that the agreement level is high [7].
\end{comment}


\begin{comment}
This process involves 3 phases and was performed by the first two authors of this paper:
• Phase I: The first two authors manually check 50 rollbacks from the 369 sampled rollbacks and generate 13 manually-derived reasons (listed in Table 3). To better understand the reasons behind rollbacks, we also look at the comments and the revisions after a rollback.
• Phase II: The first two authors independently applied the derived reasons of Phase I to categorize all 369 sampled rollbacks. They took notes regarding the deficiency or ambiguity of the reasons for categorizing certain rollbacks. Cohen’s kappa [13] is calculated to measure the inter-rater agreement and the value is 0.87, which implies a high level of agreement.
• Phase III: The first two authors discussed the categorizing results obtained in Phase II to revolve the disagreements until a consensus was reached. No new reasons were added during this discussion.
\end{comment}

\phead{Approach.} We conduct a manual study by analyzing all the duplicate logging statements in the studied systems. In total, we studied \peter{X} \zhenhao{X = sets of all the dup log or sets that belong to a pattern?} \peter{all sets}set of duplicate logging statements (i.e., each set contains two or more logging statements with the same static message). 

The process of our study involves five phases: 

\begin{itemize}
	\item Phase I: The first two authors manually studied 289 randomly sampled (based on 95\% confidence level and 5\% confidence interval~\cite{boslaugh2008statistics}) sets of duplicate logging statements and the surrounding code to derive an initial list of duplicate logging code smell patterns. All disagreements were discussed until a consensus was reached. \zhenhao{What if the lists generated by the two authors are different?} \peter{changed a little}%The authors studied all of the static messages, log levels, and surrounding code/comments to derive the patterns. 
	\item Phase II: The first two authors {\em independently} categorized {\em all} duplicate logging statements based on the derived patterns in Phase I. We did not find any new pattern in this phase. 
	\item Phase III: The first two authors discussed the categorizing results obtained in Phase II. All disagreements are discussed until a consensus was reached. 
	\item Phase IV: The first two authors further studied all code smell instances that belong to each pattern in order to identify justifiable cases of the code smell that may not need refactoring.
	\item Phase V: We verified the code smell instances and justifiable cases with the developers. 
\end{itemize}





%To uncover patterns of duplicate logging code smells, we follow a lightweight open coding-like process to identify the patterns in which the duplicate log belongs~\cite{seaman1999qualitative}. Namely, the first two authors independently go through the 


%we first go through the sampled sets of duplicate logs to uncover possible code smell patterns. We iterate the process until no new patterns emerge.  


%randomly sampling a total of 289 sets of duplicate logs (based on 95\% confidence level and 5\% confidence interval~\cite{boslaugh2008statistics}). Since the number of duplicate logs varies significantly across the studied systems, similar to prior studies~\cite{log_pattern_ICSE2017, boslaugh2008statistics}, we use the stratified sampling technique. We calculate the sample size according to the number of duplicate logs in each studied system. As an example, we detected a total of 1,168 sets of duplicate logs (i.e., each set contains two or more logs with the same message) in all the studied systems, and 865 of them are in CloudStack (74\%). Therefore, we sample $74\% * 289 = 213$ sets of duplicate logs from CloudStack. Similarly, we detected 217, 46, and 40 sets from Hadoop, Cassandra, and ElasticSearch, and we sampled 54, 12, and 10 sets, respectively. To uncover patterns of duplicate logging code smells, we follow a lightweight open coding-like process to identify the patterns in which the duplicate log belongs~\cite{seaman1999qualitative}. Namely, we first go through the sampled sets of duplicate logs to uncover possible code smell patterns. We iterate the process until no new patterns emerge. %Our first goal is to manually derive the categories of the causes. 




\begin{table*}
\caption{Patterns of duplicate logging code smells 
and corresponding examples.} %\ahmed{nothing about parallel development or is that showing up as a theme throughout the different challenges?}
\centering
%\resizebox{\textwidth}{!} {%
%\begin{adjustbox}{width=1\textwidth}

\begin{tabular}{m{.2\textwidth} | m{.65\textwidth}  }%{ m{3cm} |l}
\toprule
\textbf{Name} & \textbf{Example} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%This example is from Cloudstack, com.cloud.api.dispatch.ParamProcessWorker.processParameters
Inadequate information in catch blocks (IC) & 
\includegraphics[width=0.65\textwidth]{figures/manual_IC}

\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%This example is from Cloudstack
Inconsistent error diagnostic information (IE) & \includegraphics[width=0.65\textwidth]{figures/manual_IE}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%This is from CloudStack
Log message mismatch (LM) & \includegraphics[width=0.65\textwidth]{figures/manual_M}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
%This is from Cassandra, same class: CompactionManager 
Inconsistent log level (IL) & \includegraphics[width=0.65\textwidth]{figures/manual_L}
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
%This example is from Hadoop
Duplicate log in polymorphism  (DP) & \includegraphics[width=0.65\textwidth]{figures/manual_DI}
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bottomrule
\end{tabular}
%}
%\end{adjustbox}
\label{tab:patterns}
\end{table*}

\phead{Results.} In total, we uncovered five patterns of duplicate logging code smells. Table~\ref{tab:patterns} lists the uncovered patterns of duplicate logging code smells and the corresponding examples. Below, we discuss each pattern according to the following template: 


\begin{LaTeXdescription}
  \item[{\em Description:}] A description of the pattern of duplicate logging code smell. 
  \item[{\em Example:}] We discuss an example of the pattern.
  \item[{\em Justifiable cases:}] \peter{maybe just copy what we have to here. I feel we need to discuss both problematic and justifiable cases here. }
  \item[{\em Developers' Feedback:}] We give a summary of developers' feedback on both the problematic and justifiable cases.

\end{LaTeXdescription}



%\phead{Patterns of duplicate logging code smells.}
%In total, we uncovered five patterns of duplicate logging code smells. Table~\ref{tab:patterns} lists the uncovered patterns of duplicate logging code smells and the corresponding examples. Below, we describe each pattern in detail and discuss its potential problems. Note that these uncovered patterns are indications of potential problems. We use these patterns as a starting point to find more instances of duplicate logging code smells. For the duplicate logs that do not belong to one of the five patterns, we find that they are likely not a problem and are excluded in further studies. 

%In Section~\ref{sec:userstudy}, we further conduct a detailed manual analysis on the problematic cases (i.e., require refactoring) and justifiable (i.e., does not require refactoring) cases of each uncovered pattern. 

\peter{Zhenhao, can you please, for each pattern, copy what we have and make each pattern follow the template?}
\phead{Pattern 1: Inadequate information in catch blocks (IC).} 

\noindent{\bf {\em Description. }}Developers usually rely on logs for error diagnostics when exceptions occur~\cite{Yuan:2014:STP:2685048.2685068}. However, we find that sometimes, duplicate logs in the {\em catch} block of different exceptions may cause debugging difficulties since the logs fail to tell which exception occurred. 

\noindent{\bf {\em Example. }}As shown in Table~\ref{tab:patterns}, in the {\tt\small ParamProcessWorker} class in CloudStack, the {\em try} block contains two {\em catch} blocks; however the log messages in these two {\em catch} blocks are identical. Since both the exception message and stack trace are not logged, once one of the two exceptions occurs, developers may encounter difficulties in finding the root causes and determining the occurred exception. 

\noindent{\bf {\em Justifiable cases. }}

\phead{Pattern 2: Inconsistent error diagnostic information (IE).} 
\noindent{\bf {\em Description. }}We find that sometimes duplicate logs may contain inconsistent error diagnostic information. Namely, the recorded dynamic variables are different (e.g., one log records the stack trace but the other log does not), even though the surrounding code is very similar. 

\noindent{\bf {\em Example. }}As shown in Table~\ref{tab:patterns}, the two classes {\tt\small Create\textbf{PortForwarding}RuleCmd} and {\tt\small Create\textbf{Firewall}RuleCmd} in CloudStack have similar functionality. The two logging statements have the same static text message and are in methods with identical names (i.e., {\em create()}, not shown due to space restriction). The two {\em create()} methods have very similar code structure and perform very similar functionalities. The {\em create()} method in {\tt\small Create\textbf{PortForwarding}RuleCmd} is about creating rules for port forwarding and the method in {\tt\small Create\textbf{Firewall}RuleCmd} is about creating rules for firewalls. However, the two logging statements record different information: One records the stack trace information and the other one only records the exception message (i.e., {\em ex.getMessage()}). Due to the similar context of the two logging statements, the error diagnostic information that is recorded by the logs may also need to be consistent (we reported this problem to developers and it is now fixed as we suggested). 

\noindent{\bf {\em Justifiable cases. }}








\phead{Pattern 3: Log message mismatch (LM).} We find that sometimes after developers copy and paste a piece of code, they may forget to change the log message. As an example, in Table~\ref{tab:patterns}, the method {\em doScaleDown()} is a clone of {\em doScaleUp()} with very similar code structure and minor syntactical differences. However, developers forgot to change the log message in {\em doScaleDown()}, after the code was copied from {\em doScaleUp()} (i.e., both log messages contain {\em scaling up}). The problem causes confusion when developers analyze the logs. 


\phead{Pattern 4: Inconsistent log level (IL).} Log levels (e.g., {\em fatal}, {\em error}, {\em info}, {\em debug}, or {\em trace}) allow developers to specify the severity of the log message and to reduce logging overhead when needed (e.g., {\em debug} is usually disabled in production)~\cite{Li2017}. A prior study~\cite{Yuan:2012:CLP:2337223.2337236} shows that log level is frequently modified by developers in order to find the most adequate level. We find that there are duplicate logs that, even though the log messages are exactly the same, the log levels are different. As shown in Table~\ref{tab:patterns}, the two methods are both from the class {\tt\small CompactionManager} in Cassandra. The two methods have very similar functionality (i.e., both try to perform cleanup after compaction), but we find that the log levels are different in these two methods. 


\phead{Pattern 5: Duplicate log in polymorphism (DP).} Classes in object-oriented languages are expected to share similar functionality if they inherit the same parent class or if they implement the same interface (i.e., polymorphism). Since log messages record a higher level abstraction of the program~\cite{Shang:2014:ULL:2705615.2706065}, we find that even though there are no clones among a parent method and its overridden methods, such methods may still contain duplicate logs. Such duplicate logs may cause maintenance overhead. For example, when developers update one log message, he/she may forget to update the log message in all the other sibling classes. Inconsistent log messages may cause problems during log analysis~\cite{mehran_emse_2018, HADOOP-4190}. As shown in Table~\ref{tab:patterns}, the two classes ({\tt\small PowerShellFencer} and {\tt\small ShellCommandFencer}) in Hadoop share similar behaviors, and both classes extend the same parent class and implement the same interface. The log lines in both classes have the identical message in the inherited method. However, as systems evolve, developers may not always remember to change the log lines in both methods, which may cause problems during system debugging, understanding, and analysis.  

\hypobox{We uncovered five patterns of duplicate logging code smells based on our manual study on a statistical sample of duplicate logs.}







